Towards an Operational Responsible AI Framework for Learning Analytics in Higher Education

Universities are increasingly adopting data-driven strategies to enhance student success, with AI applications like Learning Analytics (LA) and Predictive Learning Analytics (PLA) playing a key role in identifying at-risk students, personalising learning, supporting teachers, and guiding educational decision-making. However, concerns are rising about potential harms these systems may pose, such as algorithmic biases leading to unequal support for minority students. While many have explored the need for Responsible AI in LA, existing works often lack practical guidance for how institutions can operationalise these principles. In this paper, we propose a novel Responsible AI framework tailored specifically to LA in Higher Education (HE). We started by mapping 11 established Responsible AI frameworks, including those by leading tech companies, to the context of LA in HE. This led to the identification of seven key principles such as transparency, fairness, and accountability. We then conducted a systematic review of the literature to understand how these principles have been applied in practice. Drawing from these findings, we present a novel framework that offers practical guidance to HE institutions and is designed to evolve with community input, ensuring its relevance as LA systems continue to develop.

==> sections/rai_principles_and_LA_studies_backup.tex <==
We address in this section the third research question \textit{(RQ3): How have previous Learning Analytics studies incorporated Responsible AI principles in practice?} To answer this, we conducted a systematic literature review of relevant studies in LA within HE. Our focus was on identifying works that address ethical concerns, incorporate responsible practices, and provide technical and operational solutions, as well as lessons learned from implementation.

\subsection{A Systematic Literature Review}

We initiated our systematic literature review by identifying key terms derived from our research questions and the ethical principles discussed (see Table~\ref{tab:common-principles}). We compiled a list of synonyms to create a comprehensive search string using Boolean operators (AND, OR). The structured search query was formulated as follows: \{domain of interest\} + \{area of implementation\} + \{principles\} + \{focus\}. The resulting search string was defined as \textit{('learning analytics' OR 'predictive learning analytics') AND ('higher education') AND (fairness OR transparency OR privacy OR accountability OR safety OR explainability OR ethics OR 'responsible AI') AND (framework OR guideline OR policy OR 'code of practice' OR principles OR 'best practice' OR implications OR 'lessons learn')}. 

This search string was applied across three digital libraries—ERIC, SCOPUS, and ACM—selected for their relevance to our study. Searches were conducted on titles, abstracts, and keywords. Table~\ref{tab:lit-search-results} presents the number of results obtained from each library. Before selection, we removed duplicate results. Subsequently, we established robust inclusion and exclusion criteria based on our research questions (see Table~\ref{tab:literature-criteria}). We focused on studies that explore the responsible adoption of Learning Analytics (LA) in Higher Education. This included papers detailing lessons learned from LA implementations, identifying challenges faced by UK Higher Education Institutions (HEIs), and proposing strategies to address these issues, such as policy and guideline development.



% =============== TABLE STARTS
\begin{table}[]
\centering
\caption{Literature search results}
\label{tab:lit-search-results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{llc}
\hline
\textbf{Digital library}                    & \textbf{URL}                                & \multicolumn{1}{l}{\textbf{Search results}} \\ \hline
ERIC Education Resources Information Center & \url{https://eric.ed.gov/} & 54                                          \\
Scopus              & \url{https://www.scopus.com} & 70  \\
ACM Digital Library & \url{https://dl.acm.org}     & 110 \\ \hline
\end{tabular}%
% }
\end{table}
% =============== TABLE ENDS



% =============== TABLE STARTS
\begin{table}[]
\centering
\caption{Inclusion and exclusion criteria}
\label{tab:literature-criteria}
\begin{tabular}{ll}
\hline
\multicolumn{2}{l}{\textbf{Inclusion criteria}}                \\ \hline
1 & Studies that describe ethical concerns in the adoption LA or PLA by HEI \\
2 & Studies that describe ethical challenges or address specific ethical principles for adoption of LA  \\
3 & Studies that discuss, suggest or have implemented controls, guidelines or policies for ethical adoption of LA.  \\ \hline
\multicolumn{2}{l}{\textbf{Exclusion criteria}}                \\ \hline
1 & Studies written in a language other than English           \\
2 & Conference abstracts and editorials                        \\
3 & Studies that do not meet any of the inclusion criteria     \\ 
4 & Studies that focus on other education organisations other than HEI \\ \hline
\end{tabular}
\end{table}
% =============== TABLE ENDS

The study selection followed a three-stage process: (a) reviewing the titles and abstracts, (b) reading the introductions and conclusions, and (c) evaluating the full text. At each stage, documents were categorised into three groups: 'important,' 'unsure,' and 'not relevant.' Papers classified as 'unsure' were reviewed collectively by all authors to reach a final decision. Additionally, we employed a snowballing technique to manually include certain papers identified through key citations.

A total of 234 articles were initially identified through database searches. After removing duplicates (N=37), 197 articles proceeded to the three-stage selection process. Ultimately, 167 studies were excluded, and 30 were selected. An additional 5 studies were manually added, resulting in a final total of \todo{35} studies for this literature review. 

\subsection{Findings}

The publication years of the selected papers range from 2013 to 2024. There has been an increase in studies over the past five years, with 23 papers published since 2019, compared to 13 published prior to that. The selected studies include journal articles, book chapters, and conference papers.

To analyse how Responsible AI principles have been integrated into the literature, we first classified the selected works according to the seven principles identified in Section~\ref{sec:existingRAI}. The classification was done in two steps: (a) reading the titles and abstracts to identify the potential Responsible AI principle(s) addressed by each study, and (b) reviewing the full text, with a focus on the methodology, results, and discussion sections, to determine the primary and secondary principles covered. As shown in Table~\ref{tab:papers-by-principle}, 50\% of the analysed studies primarily focus on Privacy. The second most commonly addressed principle is Transparency. We also created a 'Various principles' category for works that discuss more than two principles. \todo {I can't see this on the table} 

In the following section, we review the selected works, discussing how they have applied Responsible AI principles in practice, the challenges encountered, and the lessons learned.
% Additionally, we include recommendations and approaches presented in Section~\ref{sec:existingRAI} and apply them to our domain or study.

% We also identified that Privacy and Transparency are two principles that are commonly discussed together in the literature?


% =============== TABLE STARTS
% \begin{table}[]
% \caption{List of principles and total of studies that touch each topic}
% \label{tab:papers-by-principle}
% \begin{tabular}{lcc}
% \hline
% \multicolumn{1}{c}{\textbf{Principle}} & \textbf{Primary principle} & \textbf{Other relevant principle} \\ \hline
% Privacy                                & 18                  & 5                        \\
% Transparency                           & 6                   & 6                        \\
% Fairness and bias                      & 3                   & 2                        \\
% Accountability                         & 3                   & 0                        \\
% Safety                                 & 1                   & 2                        \\
% Security                               & 1                   & 0                        \\
% Explainability                         & 1                   & 0                        \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[h!]
\caption{Distribution of Studies Across Responsible AI Principles}
\label{tab:papers-by-principle}
\centering
\begin{tabular}{lccccccc}
\hline
\textbf{Focus}       & \textbf{Privacy} & \textbf{Transparency} & \textbf{Fairness/Bias} & \textbf{Accountability} & \textbf{Safety} & \textbf{Security} & \textbf{Explainability} \\ \hline
Primary              & 18               & 6                     & 3                      & 3                       & 1               & 1                & 1                       \\
Secondary            & 5                & 6                     & 2                      & 0                       & 2               & 0                & 0                       \\ \hline
\end{tabular}
\end{table}
% =============== TABLE ENDS

% Lesssons learnt by principles

% Short definition for Transparency, Privacy, Responsibility can be found in \cite{Cerratto-Pargman_McGrath_2021}
\subsubsection{Accountability}
% Other ethical principles closely related to Accountability: Transparency, Interpretability and Explainability
% Lessons learn, challenges, considerations, opportunities, addressing issues
As described in the previous section, the accountability principle refers to ensuring that institutions take responsibility for the decisions produced or assisted by predictive analytics systems. 
% As with any other ethical principle, accountability should be part of the entire cycle of LA systems. 
Stakeholders (HEI directors, managers, data scientists, and developing teams) should understand their specific responsibilities throughout the entire life cycle of LA systems. 
For instance, a study by \cite{Patterson_York_Maxham_Molina_Mabrey_2023} collected feedback from students, staff and teachers as part of an LA implementation case study. Their study highlights the importance of accountability at design phase and in particular regarding data management.  
A study by \cite{Alzahrani_Tsai_Aljohani_Whitelock-wainwright_Gasevic_2023} conveys how lack of governance policies affects trust in LA systems. 
In their study, the authors collect views on trust from teachers' perspectives. In particular, a lack of clear data management policies could lead to distrust in LA systems outcomes. 
Other essential aspects of accountability include data selection and outcome monitoring, which are important to prevent bias and ensure fair outcomes. 
Additional support for defining the areas of responsibility comes from \cite{Veljanova_Barreiros_2022}. In their work, authors discuss accountability from a technical perspective and propose a list of operational criteria and few examples of evaluation indicators. For instance, an approach for transparent allocation of roles and duties include tasks such as: create a communicate clear documentation or roles and duties addressed to developers (important during design and implementation of LA) and users of LA dashboards.  
% Work by \cite{Veljanova_Barreiros_2022} describes a list of criteria applicable to the accountability principle. For instance, the authors list key elements such as legal compliance, oversight mechanisms and role allocation. 
In terms of compliance, GDPR - Recital 79 explicitly states the allocation of roles and defines the concepts such as controller, processor and data subject.
We observed that a distinction is made on how accountability as responsibility is addressed. On the one hand, when there is a sense of responsibility as a duty it is called forward-looking responsibility. It usually involves the identification of relevant stakeholders, roles, and tasks that must be allocated. On the other hand, backward-looking responsibility, related with the moral action to acknowledge LA systems outcomes. Clearly, establishing a moral responsibility to humans and systems is a complex and difficult process. 
The analysis of the literature suggest that adopting operational actions to address accountability is complex and maybe one of the most important challenge for HEI. 
This principle significantly overlaps with principles such as Safety, Security and Transparency \cite{Reidenberg_Schaub_2018}. For instance, implementing audit measures (mechanisms to inspect what, how, why predictions and automated decisions were made) could not only improve algorithmic explainability but also support who (developers, admin staff, users) can be held accountable.

 

% To consider \cite{Agarwal_Mishra_2021} Chapter 7

\subsubsection{Safety}
% What is safety? why is important/what have we learn? how to me implement?
The Alan Turing Institute guideline for safe AI systems \cite{Lesli-alan-turing_2019} lists accuracy, reliability and robustness as technical characteristics for AI systems to function safely and prevent damaging outcomes. 
% not to produce damaging outcomes. 
% Translated to the domain of LA, data, decision algorithms, applications (EAS dashboards, alert systems, apps) should be designed, deployed and monitored observing these qualities. 
Translated to the domain of LA, components such as data, decision algorithms, and applications (EAS dashboards, alert systems, apps) should be designed, deployed and monitored to ensure errors are minimised (when training or processing data), any software component behaves as expected (aligned to core LA goals but also considering unexpected circumstances) and trustworthy predictions.

% In what follows, we describe recommended technical actions to improve safety in LA. 
Possible damages caused by LA could be minimised \cite{Howell_Roberts_Seaman_2018} by providing end users (students, academic staff and administrators) with clear documentation regarding the expected responsible use of LA systems (for instance, how to interpret data, good practices to contact students at risk). 
Other examples include providing conceptual clarity, proposed intent and good use guidelines of the LA system to developers \cite{Tabassi-NIST_2023}. 
Another important aspect is reliability in decision algorithms, where measurable goals for accuracy and expected model performance should be set. Considerations regarding error rate (false negatives) or accuracy level should be established. % as well as acceptable errors. 
It is important to note that many factors can influence predictions, such as, the type of machine learning algorithms, missing or incomplete features, changes in data, data noise and errors, thus setting checkpoints for training and test data are advised \cite{microsoft_2022}. 
Data accuracy plays an important role when training decision algorithms; \cite{Prinsloo_Slade_2013} analyses two HEI LA policies and reflects on the importance of putting in place policies to obtain up-to-date data from students as a way to avoid unreliable predictions that could cause damage to students and diminish trust in LA systems.

% The robustness of the systems is tested by the ability of detecting and even mitigating unexpected outcomes.

% \cite{Drachsler_Greller_2016}
% Compilation of concerns and ethical issues collected as result of a series of workshops conducted by the Learning Analytics Community Exchange, an EU project about LA

% The study is focused on data and how it should be processed fairly and lawfully;
% • accurate and up to date;

% \cite{Dixon_2023} Safety and compliance, section 4.4.


\subsubsection{Security}
% Related to the Safety principle.
It includes the implementation of technical, administrative and physical controls to mitigate risks and prevent information assets from being accidentally or deliberately compromised.
% three fundamental features confidentiality, integrity, and availability of information assets. 
Controlling access to students' and tutors' data (confidentiality), avoiding data alteration and deletion (integrity), and ensuring (authorised users) timely access to LA systems (availability) are crucial. 

As observed in the literature, researchers are concerned about security from two particular angles: privacy and data security \cite{Eleni_2023}. 
% Understandably, any possibility that students' privacy is in danger could harm all stakeholders involved. 
This is because education institutes collect a wide range of socio-demographic data from students (for example, gender, age, ethnicity, education, occupation, disability, index of multiple deprivation and country), as well as student progress data such as weekly activity in virtual learning environment systems; any possibility of this data being leaked could be damaging for students as well as HEI. 
In particular, personal and sensitive data acquisition, processing, storage and eventual disposal are heavily dependent on legal and regulatory compliance \cite{Karunaratne_2021}. 
Precisely, the General Data Protection Regulation (GDPR) describes the 'security principle' as the process of personal data \textit{securely by means of ‘appropriate technical and organisational measures’}. 

In the literature, \cite{Skene_Winer_Kustra_2022} compiles a set of considerations for ethical data governance; it includes aspects of data security such as data process (public, sensitive, personal, and high-risk), storage (local or remote) or audit plans, among others. 
Furthermore, there are organisations such as the Information Commissioners' Office (ICO) that have made available an GDPR action checklist\footnote{ICO - \url{https://ico.org.uk/for-organisations/uk-gdpr-guidance-and-resources/security/a-guide-to-data-security/}} for organisations to be aware and implement security controls. This set of tasks can be easily implemented in LA systems.

We also observe that studies focus mostly on legal-based solutions, describe data security concerns or highlight the importance of security, however, specific operational and technical controls are still lacking; understandably, these should be tailored according to organisations' goals and technological resources, and evolve as technology changes.
% Securing LA systems requires the identification of risks and the management of risks, and while recognised international standards, such as ISO 27001, are used for a holistic approach to security; data, in particular personal and sensitive data, its acquisition, processing, storage and eventual disposal, is subject to legal and regulatory controls, GDPR is an example of such regulations.
% , in particular when students personal and sensitive data is used by HEI. 

% Article 5(1)(f) of the UK GDPR concerns the ‘integrity and confidentiality’ of personal data. It says that personal data shall be:

%     'Processed in a manner that ensures appropriate security of the personal data, including protection against unauthorised or unlawful processing and against accidental loss, destruction or damage, using appropriate technical or organisational measures'


% , this digital assets should be secured against any unauthorised access, theft,  


% \cite{Lawson_Beer_Rossi_2016} check if need to delete


\subsubsection{Fairness and bias} 

Fairness and bias have gained significant attention in the LA community, with dedicated workshops like FairLAK\footnote{\url{https://sites.google.com/view/fairlak}} addressing the topic. Studies have highlighted the need to assess LA algorithms for biases and implement mitigation measures\cite{rets2023six}. Working towards this direction, some works examine fairness metrics, such as error distribution across student demographics, to determine bias against specific groups, like minority ethnic students \cite{bayer2021learning} Going a step further, Deho and colleagues\cite{deho2022existing} moved from bias detection to bias mitigation and performed a comparative evaluation of a set of selected bias mitigation approaches. The results of these studies highlight that fairness does not have a universal definition and that selecting a definition of fairness is the first critical step in deciding which mitigation strategies to apply. Both of these works also show that improving fairness in LA systems doesn’t always compromise predictive performance. \cite{rets2023six} advocate for the de-weighing or removal of sensitive attributes (and potential attributes that can act as proxies - e.g., socio-economic status acting as proxy for ethnicity) from the training for PLA algorithms. However, Deho and colleagues \cite{deho2022should} show that only if a protected attribute is correlated with the target label and proves to be an important feature, then their inclusion or exclusion would affect the performance and fairness of the LA system. It is also important to consider that LA models that behave in fair manner based on past data may not behave fairly when dealing with current/future data. Deho and colleagues therefore recommend ensuring that LA models are robust to dataset drifts before deployment\cite{deho2024past}. On a recent survey of biases in education \cite{li2023moral} Li and colleagues highlighted the need to consider intersectionality (i.e., multiple sensitive attributes such as gender and ethnicity interacting together) when assessing LA algorithmic bias. They also highlighted that potential harms may arise when fairness metrics are used in unfit tasks, leading to reach a false conclusion and thus harmful decisions are made.  Moving to the social aspect of fairness, \cite{tsai2021more} made use of questionnaires to understand, from students and staff, the implications of biases in the decision-making processes affecting these two groups. students highlighted concerns about bias perpetuation (students being labelled by data) and fear of unfair assessment due to the bias. Staff members highlighted concerns about decisions made about them based on LA ( i.e., managers who may use LA as a performance appraisal tool)


% To consider \cite{Agarwal_Mishra_2021} Chapter 2 and 3

% NIST \cite{Schwartz_Vassilev_Greene_2022} -> title: Towards a standard for identifying and managing bias in artificial intelligence
% identifies three categories of bias in AI — systemic, statistical, and human — and describes how and where they contribute to harm;
% describes three broad challenges for mitigating bias — datasets, testing and evaluation, and human factors — and introduces preliminary guidance for addressing them.


\subsubsection{Transparency} 
As mentioned in our description transparency refers to the fact that all roles involved within an LA system, from students, to staff, to other relevant stakeholders are informed. Many existing studies highlight the need to be transparent \cite{Mahrishi_Abbas_Siddiqui_2024, Tzimas_Demetriadis_2021, Cerratto-Pargman_McGrath_2021}, but do not provide practical guidance on how to do it. \cite{Drachsler_Greller_2016} emphasises the complexity in the data collection and algorithmic processes behind LA and points out that it is not trivial to provide non-technical educational stakeholders (learners, teachers, managers, education authorities or parents) with an understanding of how and what data are being collected, how they are processed, and how reliable the results of the analysis are. In this paper they advocate for playing analytics results back to the data subject and letting them decide for themselves, whether to ask for pedagogic support an intervention or not, putting the learner in control. This paper also highlights the need to obtain consent before the data collection, by finding clear and understandable consent questions (yes/no) options, and by offering the possibility to opt-out from the data collection without consequences. Hakami \cite{hakami2020learning} reviewed 37 LAK papers mentioning LA and Transparency. They highlighted the need to ensure stakeholders know how the algorithm works (algorithmic transparency), the need to set policies that reveal what data is collected and how they are used (institutional transparency), the need to inform learners that they are being tracked (transparency and data). They also highlight that transparency can enhance understanding, sense-making and reflection, technology acceptance and adoption and trust. They also highlighted the importance of given the students too opt-out, the importance of transparency from the moment of co-creating LA systems. \cite{tsai2020privacy} also highlighted the need of communication to ensure transparency. In the following work researchers aimed at operationalising transparency by proposing different technical design features of LA systems \cite{veljanova2023operationalising}






\subsubsection{Privacy}

A wide range of studies have considered the privacy implications of LA. 


2018
(Clarke, 2018)
Guidelines for the responsible application of data analytics
The Guidelines are of particular relevance to personal data
A set of Guidelines is presented, whose purpose is to intercept ill-advised uses of data and analytical tools, prevent harm to important values, and assist organisations in extracting the achievable beneﬁts from data



\subsubsection{Explainability}

\cite{Phillips_Hahn_Fontana_2021} Four principles of explainable artificial intelligence
To consider \cite{Agarwal_Mishra_2021} Chapter 4







\textcolor{red}{A paragraph to discuss that principles are not discussed in isolation, but overlapping}
2023
(Rets et al., 2023)
Six Practical Recommendations Enabling Ethical Use of Predictive Learning Analytics in Distance Education
A review of 10 publications linked to the OUAnalyse work
From the point of view of tutors, how to support them when using LA dashboards. Recommendations:
Engage the end users in the design and use of LA tools
Make LA inclusive by considering diverse student needs
Act upon LA data and communicate the added value of adopting LA tools
Use LA data to benefit students and develop an effective intervention infrastructure
Test LA data for hidden bias by engaging with diverse stakeholders

Also important a few lines about the considerations of these principles during the entire LA life cycle, including relevant stakeholders according to each stage in LA development. Without leaving behind technology aspects

2019
(Scheffel et al., 2019) 
Policy Matters: Expert Recommendations for Learning Analytics Policy
A survey with experts in the LE community. The outcome is a list of the aspects to address in LA policy “…existing policies and guidelines tend to focus on ensuring ethical and legally compliant conducts, while giving relatively little attention to other dimensions that are equally important to LA deployment…”


2021
(Cerratto Pargman and McGrath, 2021)
Mapping the Ethics of Learning Analytics in Higher Education: A Systematic Literature Review of Empirical Research
systematic literature review of the research on ethical issues that have been empirically approached in the learning analytics literature












==> sections/soa_alba_backup.tex <==
% Content
% \begin{itemize}
%     \item Query libraries to other papers in RAI. Scholarly dbs, filtered based on, increased based on industry and academy
%     \item comparative analysis on the existing frameworks, what is applicable to HE?
%     \item Analysis of RAI frameworks at the general level/industry
%     \item Analysis of frameworks in UK HEI and applied to LA
%     \item Having a comparative table, things that are missing, that are applicable, informs the framework development
% \end{itemize}

% three sections

This section describes the process for investigating the current state regarding adopting responsible AI practices, specifically when implementing Learning Analytics systems in HE. 
We gather evidence of current frameworks for responsible AI and proof of current challenges and ethical principles that higher education institutions face when adopting learning analytics systems. 
In what follows, we describe in detail the steps taken to answer our research questions. 


\subsection{Methodology}

Guided by our research questions, our approach is divided into two main phases: a) an initial exploration, investigating the latest responsible AI frameworks being used in the domain and b) a literature review to collect the ethical and social considerations of importance for UK HEI when implementing Learning Analytics (LA) systems. 
Our process follows a [recommendation or methodology]... to identify and evaluate available scientific literature relevant to Responsible AI implementation of LA and the guiding ethical principles that should be included in our framework. 

\subsubsection{Initial exploration}


We start our search by collecting information about initiatives that aim to develop, adopt or deploy AI ethically, safely, and responsibly. 
The search included frameworks approaching the ethical use of data and software development addressing the key legal, and social issues likely to arise when adopting AI systems. 
We included initiatives by well-known organisations such as Microsoft, Amazon, and Google, among others. 
We also consider policies, guidelines and codes of practice developed by Higher Education Institutions or organisations directly involved in the education domain (e.g., The Open University or JISC).
% well-known frameworks published by organisations dedicated to developing and distributing technology and software linked to the domain. 

As detailed in Table~\ref{tab:compilation-known-frameworks} we identified eleven relevant initiatives launched by organisations in different domains. 
These frameworks describe ethical and social considerations that should be given attention in every stage of the delivery of any AI technology, while providing guidance and mechanisms for responsible innovation. 
We include documents describing efforts towards an ethical practice of AI, covering principles applicable for research and development of AI technology including but not limited to, machine learning (ML), generative AI (GenAI) and any AI-powered products \cite{Google_2023,microsoft_2022, Lesli-alan-turing_2019, IBM, amazon_na}. 
Other initiatives \cite{jisc_code_2023,ou_policy_2023, Slade_Tait_icde-2019, UoE_2017}, namely code of practices, policies and guidelines, were also incorporated in our search, specifically documents focus on ML, LA and PLA design and implementation (refer to column \textit{Focus} in Table~\ref{tab:compilation-known-frameworks}).  


% As shown in Table~\ref{tab:compilation-known-frameworks} we observed that most frameworks focus on adopting AI systems from a holistic point of view, for instance, mentioning machine learning algorithms and large-scale data science technologies. Conversely, few documents address responsible AI considering specific implications for learning analytics systems adoption. 

% =============== TABLE STARTS
\begin{table}[]
\centering
\caption{Responsible AI initiatives: frameworks, guidelines, policies. AI = Artificial Intelligence, ML = Machine Learning, LA = Learning Analytics, PLA = Predictive Learning Analytics. }
\label{tab:compilation-known-frameworks}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cllcllcl}
\hline
\textbf{\#} & \multicolumn{1}{c}{\textbf{Organisation name}} & \multicolumn{1}{c}{\textbf{Document name}} & \textbf{Focus} & \multicolumn{1}{c}{\textbf{Doc. Type}} & \multicolumn{1}{c}{\textbf{Year}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ Principles\end{tabular}} & \multicolumn{1}{c}{\textbf{Context}} \\ \hline
1 & NIST & AI Risk Management Framework (NIST)~\cite{Tabassi-NIST_2023} & AI & Framework & 2023 & 7 & \begin{tabular}[c]{@{}l@{}}Non-sector-specific\\ AI development, design, \\ deployment and use\\ AI risk-oriented\end{tabular} \\
2 & Microsoft & Microsoft Responsible AI Standard~\cite{microsoft_2022} & AI & Framework & 2022 & 6 & \begin{tabular}[c]{@{}l@{}}AI in the industry\\ Product development\end{tabular} \\
3 & \begin{tabular}[c]{@{}l@{}}The Institute for Ethical\\ AI in Education - IEAIE\end{tabular} & The Ethical Framework for AI in Education~\cite{ieaie_2021} & AI & Framework & 2021 & 9 & \begin{tabular}[c]{@{}l@{}}UK\\ AI in Education\end{tabular} \\
4 & Alan Turing Institute & \begin{tabular}[c]{@{}l@{}}Understanding artificial intelligence ethics and \\ safety: A guide for the responsible design and \\ implementation of AI systems in the public sector~\cite{Lesli-alan-turing_2019}\end{tabular} & AI & Guideline & 2019 & 4 & \begin{tabular}[c]{@{}l@{}}UK\\ AI in the public sector\end{tabular} \\
5 & The Open University & Data Ethics Policy - OU (2023)~\cite{ou_policy_2023} & \begin{tabular}[c]{@{}c@{}}AI, ML, \\ Data\end{tabular} & Policy & 2023 & 4 & \begin{tabular}[c]{@{}l@{}}UK\\ The Open University\\ Data management\end{tabular} \\
6 & IBM & AI ethics at IBM~\cite{IBM} & AI & Principles description & 2024 & 5 & \begin{tabular}[c]{@{}l@{}}AI in the industry\\ Product development\end{tabular} \\
7 & Google & Google’s AI Principles~\cite{Google_2023} & AI & Principles description & 2023 & 7 & \begin{tabular}[c]{@{}l@{}}AI in the industry\\ Product development\end{tabular} \\
8 & Amazon & Building AI responsibly at AWS~\cite{amazon_na} & AI & Principles description & NE & 8 & \begin{tabular}[c]{@{}l@{}}AI in the industry\\ Product development\end{tabular} \\
9 & JISC & Code of practice for learning analytics~\cite{jisc_code_2023} & LA & Code of practice & 2023 & 7 & \begin{tabular}[c]{@{}l@{}}UK \\ Learning Analytics in HEI\end{tabular} \\
10 & \begin{tabular}[c]{@{}l@{}}ICDE - International \\ Council for Open and \\ Distance Education\end{tabular} & Global Guidelines: Ethics in Learning Analytics~\cite{Slade_Tait_icde-2019} & \begin{tabular}[c]{@{}c@{}}LA, \\ PLA\end{tabular} & Guideline & 2019 & 10 & \begin{tabular}[c]{@{}l@{}}Global\\ Learning Analytics \\ in Education\end{tabular} \\
11 & University of Edinburgh & Learning Analytics Principles and Purposes~\cite{UoE_2017} & LA & Policy & 2017 & 7 & \begin{tabular}[c]{@{}l@{}}UK\\ University of Edinburgh\\ Learning Analytics in HEI\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}
% =============== TABLE ENDS

% RESEARCH QUESTIONS!
% - What are the ethical considerations (as stated in the literature) that a responsible framework should look at when adopting learning analytics and predictive learning analytics systems by UK Higher Education Institutes
% - What are the ethical considerations (as stated in the literature) that a responsible framework should look at when adopting learning analytics and predictive learning analytics systems by UK Higher Education Institutes?

\subsubsection{Literature search strategy}

The next activity focuses on identifying the ethical considerations that represent key challenges or concerns for UK Higher Education Institutes (HEI), we are interested in legal and technical aspects but fundamentally social factors and risks when adopting learning analytics and predictive learning analytics systems. 
% UK Higher Education Institutes (HEI) when adopting learning analytics and predictive learning analytics systems and 
% The literature search process consisted of exploring current works on \texttt{responsible AI} and \texttt{frameworks} for learning analytics in the UK HEIs using Google Scholar. This helped to gain a comprehensive understanding of the latest research in the field and to devise candidate keywords and search queries. 
The literature search process consisted of exploring current works on \texttt{responsible AI} and \texttt{frameworks}, focused on 
To perform the literature search we focused on building the search query. First, we identify main terms from the initial exploration step and the findings regarding ethical principles guiding well-known organisations' adoption of responsible AI. 
In order to gain a comprehensive understanding of the latest research in the field and to devise candidate keywords and search queries. 
We stare identifying the main terms from the research questions and the findings related to the most common ethical principles guiding well-known organisations' adoption of responsible AI ethics (see Table~\ref{tab:common-principles}). 
After identifying the keywords, we compiled a list of synonyms to construct the search string using Boolean operators AND OR. The resulting search string was then defined as \textit{('learning analytics' OR 'predictive learning analytics') AND ('higher education') AND (fairness OR transparency OR privacy OR accountability OR safety OR explainability OR ethics OR 'responsible AI') AND (framework OR guideline OR policy OR 'code of practice' OR principles OR 'best practice' OR implications OR 'lessons learn')}. 
The search string was used in three digital libraries: ERIC, SCOPUS and ACM. These digital libraries were selected based on their relevance. The search was set to include a title, abstract and keywords. Table~\ref{tab:lit-search-results} shows the number of results obtained in each digital library. 
Before selecting the relevant studies, duplicate results were removed.
% ("learning analytics" OR "predictive learning analytics") AND "higher education" AND (fairness OR transparency OR privacy OR accountability OR safety OR explainability OR ethics OR "responsible AI") AND (framework OR guideline OR policy OR "code of practice" OR principles OR "best practice" OR implications OR "lessons learn")

% =============== TABLE STARTS
\begin{table}[]
\centering
\caption{Literature search results}
\label{tab:lit-search-results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{llc}
\hline
\textbf{Digital library}                    & \textbf{URL}                                & \multicolumn{1}{l}{\textbf{Search results}} \\ \hline
ERIC Education Resources Information Center & \url{https://eric.ed.gov/} & 54                                          \\
Scopus              & \url{https://www.scopus.com} & 70  \\
ACM Digital Library & \url{https://dl.acm.org}     & 110 \\ \hline
\end{tabular}%
% }
\end{table}
% =============== TABLE ENDS

\subsubsection{Study selection and quality evaluation}

As a first step in the study selection process, we established inclusion and exclusion criteria in line with our research questions. The criteria can be found in Table~\ref{tab:literature-criteria}. 
We consider the responsible adoption of LA from and institutional perspective, where ethical and social considerations are taken into account for the use of LA to support the students' learning process and tutors' activities. 
Therefore, we included papers describing lessons learnt during the adoption of LA, also papers that collect challenges and concerns faced by UK HEI and approaches to overcome such challenges, including policy and guidelines proposals as well as solutions to address specific ethical principles.


% =============== TABLE STARTS
\begin{table}[]
\centering
\caption{Inclusion and exclusion criteria}
\label{tab:literature-criteria}
\begin{tabular}{ll}
\hline
\multicolumn{2}{l}{\textbf{Inclusion criteria}}                \\ \hline
1 & Studies that present solutions for the ethical and responsible adoption of LA \\
2 & Studies that study challenges, ethical and social considerations for adoption of LA \\
3 & Studies that discuss findings regarding ethical concerns in LA       \\ \hline
\multicolumn{2}{l}{\textbf{Exclusion criteria}}                \\ \hline
1 & Studies written in a language other than English           \\
2 & Conference abstracts and editorials                        \\
3 & Studies that do not meet any of the inclusion criteria     \\ \hline
\end{tabular}
\end{table}
% =============== TABLE ENDS

The studies were selected following a three-stage process: (a) reading the titles and abstracts of the studies, (b) the introduction and conclusion and (c) the paper full text. 
At each stage, the documents were classified into three groups: 'important', 'not sure' and 'not relevant'. 
% Might delete this later
All the authors reviewed the studies classified as 'not sure' before reaching a final decision.
% Papers classified as 'not sure' were reviewed by the all the authors before reaching reaching a final decision. 
Additional papers were manually included because studies in the main search cited them or we came across them during the initial exploration phase.

A total of 234 articles were extracted by searching the databases. Duplicates were removed (N=37), therefore 197 reached the three-stage selection process. 
In total 167 studies were excluded and 30 were selected. Finally, five studies were added manually, with 35 studies considered for this literature review. 

\textcolor{red}{TODO: Appendix with the list of papers}


\subsection{Findings}

% What are the ethical considerations (as stated in the literature) that a responsible framework should look at when adopting learning analytics and predictive learning analytics systems by UK Higher Education Institutes?

% \begin{itemize}
%     \item demonstrate that their is a gap in the literature, no study has proposed a framework for adoption of responsible LA in education
%     \item demonstrate that the selected principles are important. Given the current challenges
% \end{itemize}

% \begin{itemize}
%     \item RQ1: We select works that proposed a framework (guideline, code of practice, best practices) for the responsible (considering ethical principles) adoption of learning analytics systems. 
%     \item RQ2: We select works that highlight ethical challenges in the domain, specifically, those works focusing on analysing the principles that HEI should consider when implementing learning analytics systems or predictive learning analytic systems. 
% \end{itemize}

This section reports the results by application of the methodology described previously. The findings are also discussed and serve as the fundamental resources for answering the research questions presented in Section~\ref{sec:introduction}.

\subsubsection{Responsible AI frameworks for the adoption of LA/PLA}
% RESEARCH QUESTIONS
% - What is the current status in the artificial intelligence domain with regards of responsible frameworks for the adoption of learning analytics and predictive learning analytics systems in the UK Higher Education Institutes?

To determine the current initiatives advancing efforts towards a responsible practice of AI, we analysed eleven documents, including, frameworks, guidelines, policies and code of practice. These documents have been published by organisations involved in developing AI-powered technology (for instance, machine learning and generative AI), AI research, implementation of learning analytics (LA) systems, predictive learning analytics (PLA) systems and policymakers. 
Table~\ref{tab:compilation-known-frameworks} provides a general overview of the documents published by each organisation, organised by its main focus and information about the type of document, year of publication and a number of ethical principles addressed. 

It is important to highlight that most organisations have formalised their approaches to social an ethical principles as a necessity 
acknowledge the ever-growing AI solutions
The organisations that have adopted or created 

A comprehensive review of the s
A comprehensive review of the frameworks reveals that organisations acknowledge the ever-growing of innovative solutions in AI, availability of big data, cloud computing platforms and evolving machine learning algorithms  that the design and deployment of AI systems require a collective effort  a few organisations approach specific technologies. 


For instance, the University of Edinburgh's policy \cite{UoE_2017}, the ICDE guideline \cite{Slade_Tait_icde-2019} and JISC's code of practice \cite{jisc_code_2023} focus on the adoption of LA and PLA. 
On the other hand, the majority of the frameworks approach responsible practices from a holistic point of view

However, it is important to note that not all issues discussed in each document apply to all AI systems, for instance, machine learning algorithms trained to detect spam will present less ethical challenges than one trained to identify students requiring support or early intervention with courses \textcolor{red}{improve the example}.   

,  specifically in UK Higher Education Institutions (HEI). 
Most of them approach responsible AI practices in a general 


I can talk about different things: the type of organisations, the type of documents, the type of focus, mention how up-to-date they are and finally the principles


in particular those focusing on  responsible learning analytics and predictive learning analytics systems in the UK Higher Education Institutes, 


We select works that proposed a 

The results obtained during the initial exploration 
Rephrase to indicate that there is a gap in the literature as most of them are focused on AI in 


Other initiatives \cite{jisc_code_2023,ou_policy_2023, Slade_Tait_icde-2019, UoE_2017}, namely code of practices, policies and guidelines, specifically focus on ML, LA and PLA design and implementation (refer to column \textit{Focus} in Table~\ref{tab:compilation-known-frameworks}).  

of the initial exploration regarding the latest initiatives for responsible AI. Next, the findings concerning  the literature review findings  highlighting the ethical challenges and concerns during AL implementation. 
the findings of the literature review are reported. First, presenting and analysis of the initial exploration and studies results, followed by the 




A framework in education ~\cite{Saxena_García_2023}


Clarification why SHEILA is not included "The SHEILA framework was created within the context of the EU SHEILA project [29]. The framework aims to support HEI in the LA policy development process."


Mention to SHEILA y why it was not included
\textit{SHEILA, in addition to helping in the development of institutional
policies, serves as a readiness evaluation instrument but does not provide activities to
work on the identified challenges.}

Mention to LALA and why it was not included
% The LALA framework can be considered
% the most complete since it provides a set of guidelines and instruments to support
% the adoption of LA in Latin America, although it focuses on piloting tools and does not
% focus on the dynamics of an LA team.

demonstrate that their is a gap in the literature, no study has proposed a framework for adoption of responsible LA in education

\subsubsection{Ethical considerations for a responsible AI framework in LA/PLA. }

Our analysis of the eleven documents regarding Responsible AI frameworks resulted in the observation of a shared concern across different organisations and a range of ethical considerations that most institutions face when approaching ethical practice in AI.
Clearly, only a few initiatives have proposed guidelines or policies \cite{jisc_code_2023, Slade_Tait_icde-2019,UoE_2017} to adopt ethical principles focused on of learning analytics in the education domain.

From this initial review, we also observe that these initiatives describe a set of foundational properties for ethical AI, namely \textbf{\textit{'ethical principles'}}. 
Closer inspection of these initiatives (frameworks, guidelines, policies) shows that although each organisation tailors and defines its guiding ethical principles according to its objectives and values, there is a small set of principles shared amongst all organisations (see Table~\ref{tab:common-principles}). 
The seven most common ethical principles are: Fairness and bias, Privacy, Transparency, Accountability, Explainability, Safety and Security.

Our analysis of the eleven documents regarding Responsible AI frameworks results in the observation of a shared concern across different organisations and a range of ethical considerations that most institutions face when approaching ethical practice in AI.
Clearly, only a few initiatives have proposed guidelines or policies \cite{jisc_code_2023, Slade_Tait_icde-2019,UoE_2017} to adopt ethical principles focused on of learning analytics in the education domain. 

\cite{Dixon_2023} Dixon did a study of ethical considerations and supports our findings.

\textcolor{red}{TODO: connect the idea to the next step: literature review}
These initiatives mostly address specific requirements oriented to the governance of data and the compliance of legal regulations, such as GDPR and the Data Act (UK) 

% \begin{tabular}[c]{@{}l@{}}\cite{Google_2023},\cite{jisc_code_2023},\cite{Tabassi-NIST_2023},\cite{ou_policy_2023},\cite{microsoft_2022},\\ \cite{ieaie_2021}, \cite{Lesli-alan-turing_2019},\cite{Slade_Tait_icde-2019},\cite{UoE_2017},\cite{amazon_na},\cite{IBM}\end{tabular}}

% \begin{tabular}[c]{@{}l@{}}\cite{Tabassi-NIST_2023},\cite{IBM}\end{tabular}}
% % =============== TABLE STARTS
\begin{table}[]
\centering
\caption{Most common principles. Principles in \textit{italics} indicate ...}
\label{tab:common-principles}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|llllllll}
\hline
 & \multicolumn{8}{c}{\textbf{Common principles}} \\ \cline{2-9} 
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Organisation's \\ name\end{tabular}}} & \multicolumn{1}{c}{\textbf{Fairness and bias}} & \multicolumn{1}{c}{\textbf{Transparency}} & \multicolumn{1}{c}{\textbf{Accountability}} & \multicolumn{1}{c}{\textbf{Privacy}} & \multicolumn{1}{c}{\textbf{Security}} & \multicolumn{1}{c}{\textbf{Explainability}} & \multicolumn{1}{c}{\textbf{Safety}} & \multicolumn{1}{c}{\textbf{Unclassified}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Alan Turing \\ Institute\end{tabular}} & Fairness & Transparency & Accountability & - & - & - & - & Sustainability \\
\textbf{\begin{tabular}[c]{@{}l@{}}The Open \\ University\end{tabular}} & Fairness & Transparency & Accountability & - & - & Explainability & - & - \\
\rowcolor[HTML]{EFEFEF} 
\textbf{ICDE} & Inclusion & \begin{tabular}[c]{@{}l@{}}- Communications\\ - Transparency\end{tabular} & \begin{tabular}[c]{@{}l@{}}Institutional responsibility  \\ and obligation to act\end{tabular} & \begin{tabular}[c]{@{}l@{}}- Consent\\ - Data ownership \\ and control\end{tabular} & \begin{tabular}[c]{@{}l@{}}- Accessibility of data\\ - Validity and reliability \\ of data\end{tabular} & - & - & \begin{tabular}[c]{@{}l@{}}- Cultural values\\ - Student agency and \\ responsibility\end{tabular} \\
\textbf{Google} & \begin{tabular}[c]{@{}l@{}}- Avoid creating or \\ reinforcing unfair bias\\ - Be socially beneficial\end{tabular} & - & Be accountable to people & \begin{tabular}[c]{@{}l@{}}Incorporate privacy \\ design principles\end{tabular} & - & - & \begin{tabular}[c]{@{}l@{}}Be built and \\ tested for safety\end{tabular} & \begin{tabular}[c]{@{}l@{}}- Be made available for uses that \\ accord with these principles\\ - Uphold high standards of \\ scientific excellence\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{IBM} & Fairness & Transparency & - & Privacy & Robustness & Explainability & - & - \\
\textbf{IEAIE} & Equity & \textit{\begin{tabular}[c]{@{}l@{}}- Informed Participation\\ \\ - Transparency and \\ Accountability\end{tabular}} & \textit{\begin{tabular}[c]{@{}l@{}}- Transparency and \\ Accountability\end{tabular}} & Privacy & - & - & - & \begin{tabular}[c]{@{}l@{}}- Achieving Educational Goals\\ - Administration and Workload\\ - Autonomy\\ - Ethical Design\\ - Forms of Assessment\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{JISC} & \begin{tabular}[c]{@{}l@{}}Minimising \\ adverse impacts\end{tabular} & \begin{tabular}[c]{@{}l@{}}- Transparency, legal \\ basis and consent\\ - Access\end{tabular} & Responsibility & Privacy & - Validity & - & - & - Stewardship of data \\
\textbf{\begin{tabular}[c]{@{}l@{}}University of \\ Edinburgh\end{tabular}} & \begin{tabular}[c]{@{}l@{}}- Beneficial to students\\ - Fairness and bias\end{tabular} & Transparent & \begin{tabular}[c]{@{}l@{}}Be accountable \\ to people\end{tabular} & Privacy & - & Explainability & - & - Governance \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Microsoft} & \begin{tabular}[c]{@{}l@{}}- Fairness\\ - Inclusiveness\end{tabular} & Transparency & Accountability & \textit{Privacy and Security} & \textit{\begin{tabular}[c]{@{}l@{}}- Privacy and \\ Security\end{tabular}} & - & \begin{tabular}[c]{@{}l@{}}Reliability \\ and Safety\end{tabular} & - \\
\textbf{Amazon} & Fairness & Transparency & - & \textit{Privacy and security} & \textit{\begin{tabular}[c]{@{}l@{}}- Privacy and security\\ - Veracity and robustness\end{tabular}} & \begin{tabular}[c]{@{}l@{}}- Explainability\\ - Controllability\end{tabular} & Safety & - Governance \\
\rowcolor[HTML]{EFEFEF} 
\textbf{NIST} & \begin{tabular}[c]{@{}l@{}}Fair with harmful \\ bias managed\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}- Accountable and \\ transparent\end{tabular}} & \textit{\begin{tabular}[c]{@{}l@{}}Accountable and \\ transparent\end{tabular}} & Privacy-enhanced & \begin{tabular}[c]{@{}l@{}}- Secure and resilient\\ - Valid and reliable\end{tabular} & \begin{tabular}[c]{@{}l@{}}Explainable \\ and interpretable\end{tabular} & - Safe & - \\ \hline
\end{tabular}%
}
\end{table}
% % =============== TABLE ENDS



% \begin{enumerate}
%     \item We start by exploring well-known frameworks from organisations that have developed state-of-the-art AI tools. We can mention Microsoft, Amazon, etc.
%     \item We also consider frameworks (also referred to as policies, guidelines and codes of practice) developed by Higher Education Institutions or directly involved with them; we can mention Jisc, etc.
%     \item From our analysis we could identify that these frameworks share a set of principles that set the foundation for a Responsible implementation of AI systems. In total  
%     \item  focusing on the rising interest in responsible AI and ethical concerns
% \end{enumerate}


% We start by investigating the latest frameworks in the AI domain; as a result, we identify a list of common principles guiding most of these proposals. 
% Next, we review the literature regarding initiatives focused on Responsible AI frameworks for LA, and in particular, identify pressing issues that represent ethical challenges for higher education institutions when adopting learning analytics systems. 



DEFINITIONS

Short definition for Transparency, Privacy, Responsibility can be found in \cite{Cerratto-Pargman_McGrath_2021}

\subsubsection{Fairness and bias}

To consider \cite{Agarwal_Mishra_2021} Chapter 2 and 3

\subsubsection{Transparency}

\subsubsection{Accountability}

To consider \cite{Agarwal_Mishra_2021} Chapter 7

\subsubsection{Privacy}

\subsubsection{Security}

\subsubsection{Explainability}

To consider \cite{Agarwal_Mishra_2021} Chapter 4

\subsubsection{Safety}



2023
(Rets et al., 2023)
Six Practical Recommendations Enabling Ethical Use of Predictive Learning Analytics in Distance Education

A review of 10 publications linked to the OUAnalyse work
From the point of view of tutors, how to support them when using LA dashboards. Recommendations:
Engage the end users in the design and use of LA tools
Make LA inclusive by considering diverse student needs
Act upon LA data and communicate the added value of adopting LA tools
Use LA data to benefit students and develop an effective intervention infrastructure
Test LA data for hidden bias by engaging with diverse stakeholders

2019
(Scheffel et al., 2019) 
Policy Matters: Expert Recommendations for Learning Analytics Policy
A survey with experts in the LE community. The outcome is a list of the aspects to address in LA policy “…existing policies and guidelines tend to focus on ensuring ethical and legally compliant conducts, while giving relatively little attention to other dimensions that are equally important to LA deployment…”

2018
(Clarke, 2018)
Guidelines for the responsible application of data analytics
The Guidelines are of particular relevance to personal data

A set of Guidelines is presented, whose purpose is to intercept ill-advised uses of data and analytical tools, prevent harm to important values, and assist organisations in extracting the achievable beneﬁts from data

2021
(Cerratto Pargman and McGrath, 2021)
Mapping the Ethics of Learning Analytics in Higher Education: A Systematic Literature Review of Empirical Research
systematic literature review of the research on ethical issues that have been empirically approached in the learning analytics literature

2022
(Schwartz et al., 2022)
Towards a standard for identifying and managing bias in artificial intelligence
NIST 
identifies three categories of bias in AI — systemic, statistical, and human — and describes how and where they contribute to harm;
describes three broad challenges for mitigating bias — datasets, testing and evaluation, and human factors — and introduces preliminary guidance for addressing them.






